Exploiting Variational Domain-Invariant User Embedding for Partially Overlapped Cross Domain Recommendation

Cross-Domain Recommendation (CDR) has been popularly studied to utilize different domain knowledge to solve the cold-start problem in recommender systems. Most of the existing CDR models assume that both the source and target domains share the same overlapped user set for knowledge transfer. However, only few proportion of users simultaneously activate on both the source and target domains in practical CDR tasks. In this paper, we focus on the Partially Overlapped Cross-Domain Recommendation (POCDR) problem, that is, how to leverage the information of both the overlapped and non-overlapped users to improve recommendation performance. Existing approaches cannot fully utilize the useful knowledge behind the non-overlapped users across domains, which limits the model performance when the majority of users turn out to be non-overlapped. To address this issue, we propose an end-to-end dual-autoencoder with Variational Domain-invariant Embedding Alignment (VDEA) model, a cross-domain recommendation framework for the POCDR problem, which utilizes dual variational autoencoders with both local and global embedding alignment for exploiting domain-invariant user embedding. VDEA first adopts variational inference to capture collaborative user preferences, and then utilizes Gromov-Wasserstein distribution co-clustering optimal transport to cluster the users with similar rating interaction behaviors. Our empirical studies on Douban and Amazon datasets demonstrate that VDEA significantly outperforms the state-of-the-art models, especially under the POCDR setting.

==> model.tex <==
\section{Modeling for \modelname}

\begin{figure*}
\centering
\includegraphics[width=0.95\linewidth]{pic/EXMP3.pdf}
% \vspace{-0.9cm} 
\caption{Demonstration of the general process of \modelname~and \newmodelname. (a-c) are the main processes of \modelname~while (d-f) are the main processes of \newmodelname. Notably that the preference attribution (Romantic or Realistic) is just an example and it is not directly accessible during the training process. }
\vspace{-0.5cm} 
\label{fig:insight}
\end{figure*}

First, we describe notations.
%
We assume there are two domains, i.e., a source domain $\mathcal{D}^\mathcal{S}$ and a target domain $\mathcal{D}^\mathcal{T}$.
%
We assume $\mathcal{S}$ has $|\bm{U}^\mathcal{S}|$ users and $|\bm{V}^\mathcal{S}|$ items, and $\mathcal{T}$ has $|\bm{U}^\mathcal{T}|$ users and $|\bm{V}^\mathcal{T}|$ items. 
%
% Let $\bm{R}^\mathcal{S} \in \mathbb{R}^{|\bm{U}^\mathcal{S}| \times |\bm{V}^\mathcal{S}|}$ be the source rating matrix and $\bm{R}^\mathcal{T} \in \mathbb{R}^{|\bm{U}^\mathcal{T}| \times |\bm{V}^\mathcal{T}|}$ be the target rating matrix.
%
Unlike conventional cross domain recommendation, in POCDR, the source and target user sets are not completely the same.
%
In order to measure that difference, we define the overlapped user ratio $\mathcal{K}_u = |\bm{U}^\mathcal{S} \cap \bm{U}^\mathcal{T}|/|\bm{U}^\mathcal{S} \cup \bm{U}^\mathcal{T}| = |\bm{U}^\mathcal{S} \cap \bm{U}^\mathcal{T}|/|\bm{U}|$ where $|\bm{U}^\mathcal{S} \cap \bm{U}^\mathcal{T}|$ denotes the concurrence users in both source and target domains, and $|\bm{U}^\mathcal{S} \cup \bm{U}^\mathcal{T}| = |\bm{U}|$ denotes the total number of user in source and target domains.
%
$\mathcal{K}_u = 1$ means the users are completely overlapped across domains, while $\mathcal{K}_u = 0$ means there is no overlapped user across domains.


Then, we introduce the overview of our proposed \modelname~framework.
%
The aim of \modelname~is providing better single domain recommendation performance by leveraging useful cross domain knowledge for both overlapped and non-overlapped users.
%
\modelname~model mainly has two modules, i.e., \textit{rating reconstruction module} and \textit{embedding alignment module}.
%
The rating reconstruction module establishes user embedding according to the user-item interaction on the source and target domains.
%
The embedding alignment module has two parts, i.e., \textit{local embedding alignment} and \textit{global embedding alignment}, sufficiently aligning the local and global user embeddings across domains.
%
% The prime task of \modelname~is providing better single domain recommendation performance by leveraging the cross domain useful knowledge for both overlapped and non-overlapped users. \ccc{wrong place, should be near the rating reconstruction module?} \lwm{updated}
%
The framework of \modelname~has been demonstrated in the right part of Fig.~\ref{fig:model} and we will introduce its two modules in details later.

\subsection{Rating Reconstruction Module}
%
We first introduce the rating reconstruction module of \modelname.
%
We define $\bm{X}^\mathcal{S} \in \mathbb{R}^{N \times |\bm{V}^\mathcal{S}|}$ and $\bm{X}^\mathcal{T} \in \mathbb{R}^{N \times |\bm{V}^\mathcal{T}|}$ as the user-item interactions on the source and target domains respectively, and $N$ is batch size.
%
We adopt dual autoencoder as the main architecture for accurately representing user embedding according to the rating interactions. 
%
We utilize two autoenocers in \modelname, i.e., \textit{source-based autoencoder} and \textit{target-based autoencoder}, for source and target domains, respectively. 
%
The source-based autoencoder includes the encoder $E_\mathcal{S}$ and decoder $D_\mathcal{S}$, and the target-based autoencoder includes the encoder $E_\mathcal{T}$ and decoder $D_\mathcal{T}$.
%
We obtain the source and target user embeddings by $E_\mathcal{S}(\bm{X}^\mathcal{S}) = \bm{Z}^\mathcal{S} \in \mathbb{R}^{N \times D}$ and $E_\mathcal{T}(\bm{X}^\mathcal{T}) = \bm{Z}^\mathcal{T} \in \mathbb{R}^{N \times D}$, respectively, and $D$ is the dimension of user embeddings.
%
The dual autoencoder should reconstruct the user-item interaction as $\hat{\bm{X}}_\mathcal{S} = D_\mathcal{S}(\bm{Z}^\mathcal{S})$ and $\hat{\bm{X}}_\mathcal{T} = D_\mathcal{T}(\bm{Z}^\mathcal{T})$.
%
The reconstruction loss is given as:
\begin{equation}
\myfont{
\begin{aligned}
\label{equ:recon}
L_R = \frac{1}{N} \sum_{i=1}^N  \mathcal{F}(\hat{\bm{X}}^\mathcal{S}_i, \bm{X}^\mathcal{S}_i) + \mathcal{F}(\hat{\bm{X}}^\mathcal{T}_i, \bm{X}^\mathcal{T}_i) ,
\end{aligned}
}
\end{equation}
% 
where $\mathcal{F}(\cdot,\cdot)$ denotes the cross-entropy loss.
%
Through the rating reconstruction module, the encoder and decoder can model the user-item rating interactions in corresponding domains. 
%
However, without efficient knowledge sharing between the source and target domains, the cold-start and cross-domain recommendation performance will still be seriously limited.


\subsection{Embedding Alignment Module}
%
We then introduce the embedding alignment module of \modelname.
%
The first part, i.e., \textit{local embedding alignment}, aims to align user embeddings in the source and target domains from \textit{sample-based} perspective.
%
The second part, i.e., \textit{global embedding alignment}, aligns the source and target user embedding from \textit{distribution-based} perspective.

\nosection{Local embedding alignment}
%
In order to obtain domain-invariant user embedding $Z^\mathcal{S}$ and $Z^\mathcal{T}$ through the encoders $E_\mathcal{S}$ and $E_\mathcal{T}$, the overlapped users should have the same embeddings across different domains. 
%
Therefore, we propose the sample-based local user embedding alignment method for aligning the overlapped users.
%
After that, the decoders $D_\mathcal{S}$ and $D_\mathcal{T}$ can translate the user embeddings to their corresponding source or target domains.
%
Therefore, the local user embedding alignment loss is given as:
\begin{equation}
\myfont{
\begin{aligned}
L_{LA} = \sum_{i=1}^N \sum_{j=1}^N \delta(\bm{U}^\mathcal{S}_i,\bm{U}^\mathcal{T}_j) ||\bm{Z}^\mathcal{S}_i - \bm{Z}^\mathcal{T}_j||_2^2,
\end{aligned}
}
\end{equation}
where $\delta(\cdot)$ indicates whether a user occurs simultaneously in both domains under the POCDR setting. 
%
$\delta(\bm{U}^\mathcal{S}_i,\bm{U}^\mathcal{T}_j)=1$ means the $i$-th user in the source domain has the same identification with the $j$-th user in the target domain, otherwise $\delta(\bm{U}^\mathcal{S}_i,\bm{U}^\mathcal{T}_j) = 0$.
%
This loss function drives the embeddings of the overlapped users becoming more assembled with abundant domain-invariant user characteristics.
%

However, local embedding alignment can only be applied to the overlapped users.
%
Although sample-based local embedding alignment can exploit the overlapped user domain-invariant characteristics, it cannot handle the non-overlapped users who do not have rating interactions in both domains.
%
When there are a plenty of non-overlapped users in POCDR, it will greatly weaken the model performance since there is no further constraints on the non-overlapped users who also have useful knowledge. 
%
Failing to obtain more general embedding for the non-overlapped users obstructs the knowledge transfer across domains. 


Fig.~\ref{fig:insight} shows a typical example, and Fig.~\ref{fig:insight}(a) is the initial state where user embeddings in both source and target domains are separated.
%
After adopting the local embedding alignment, the overlapped users (numbered from 1 to 6) are better aligned, as shown in Fig.~\ref{fig:insight}(b).
%
However, the embeddings of other scattered non-overlapped users still have gaps across domains. 
%
From it, we can see that local embedding alignment is helpful in exploring the domain-invariant embeddings for overlapped users but cannot solve the domain discrepancy between the large majority of non-overlapped users. 
%
Thus, the sample-based local alignment is not powerful enough when there are only few overlapped users in POCDR settings.


\nosection{Global embedding alignment}
%
Both overlapped and non-overlapped users should have domain-invariant embedding distributions. 
%
Sample-based local alignment has achieved domain-invariant user embeddings for the overlapped users.
%
However, there is still a certain domain discrepancy between the non-overlapped users across domains, as can be seen in Fig.~\ref{fig:insight}(b).
%
In order to align the non-overlapped user embedding distributions across domains, we further propose global embedding alignment to exploit the domain-invariant user embeddings for all the users.
%
% Here, global embedding alignment exploits the domain-invariant user embeddings for all the users, which aims to overcome the domain shift between the non-overlapped users who have no rating interactions across domains.
%
% \ccc{
% We first align the sample-based local user preference embeddings, that is, the overlapped users should share the domain-invariant embeddings for better modelling its characteristics.
% %
% However, the non-overlapped users don't have rating interactions across domains which makes it hard to obtain sample-based local alignment.
% %
% The both source and target user latent embedding distributions will be shifted and misaligned since the leaking constraints on aligning non-overlapped users, hurdling the knowledge transfer across domains.
% %
% Thus the sample-based local alignment is not powerful enough when there are extremely few overlapped users in POCDR settings.
% %
% Therefore, we claim that the both users including overlapped and non-overlapped should also have domain-invariant embedding distribution in the global alignment perspective.
% }
%
Specifically, we adopt mean and variance to model the latent source and target user latent distributions as $\mathbb{P}(\bm{Z}^\mathcal{S}) \sim \mathcal{N}(\bm{\Omega}(\bm{Z}^\mathcal{S}),\bm{\Sigma}(\bm{Z}^\mathcal{S}))$ and $\mathbb{P}(\bm{Z}^\mathcal{T}) \sim \mathcal{N}(\bm{\Omega}(\bm{Z}^\mathcal{T}),\bm{\Sigma}(\bm{Z}^\mathcal{T}))$ respectively, where $\bm{\Omega}(\cdot)$ denotes the mean operation and $\bm{\Sigma}(\cdot)$ denotes the variance operation and they can be calculated as $\bm{\Omega}(\bm{Z}^\mathcal{X}) = \frac{1}{N} \bm{1}_N^T\bm{Z}^\mathcal{X}, \bm{\Sigma}(\bm{Z}^\mathcal{X}) = \frac{1}{N} (\bm{Z}^\mathcal{X})^T\bm{H}\bm{Z}^\mathcal{X}$, where $\bm{H} =\bm{I}_N - \frac{1}{N}\bm{1}_N\bm{1}_N^T$ denotes the scatter projection matrix and $\mathcal{X} = \{\mathcal{S},\mathcal{T}\}$ indicates different domains.
%
Since we assume normal Gaussian distribution for users in both the source and target domains, we can adopt the 2-Wasserstein distance of different Gaussians distributions to measure the discrepancy as below:
\begin{equation}
\begin{aligned}
\label{equ:hatdw}
L_{GA} &= ||\bm{\Omega} (\bm{Z}^\mathcal{S})  - \bm{\Omega}(\bm{Z}^\mathcal{T}) ||_2^2 + ||\bm{\Sigma}(\bm{Z}^\mathcal{S}) - \bm{\Sigma}(\bm{Z}^\mathcal{T} )||_2^2\\
& = {d}_W( \mathcal{N}(\bm{\Omega}(\bm{Z}^\mathcal{S}),\bm{\Sigma}(\bm{Z}^\mathcal{S})), \mathcal{N}(\bm{\Omega}(\bm{Z}^\mathcal{T}),\bm{\Sigma}(\bm{Z}^\mathcal{T}))).
\end{aligned}
\end{equation}
%
The meaning of the global user embedding distribution alignment is aligning the mean and standard variance of all the users  across different domains. 
%
After it, the marginal probability distribution of $\mathbb{P}(\bm{Z}^\mathcal{S})$ and $\mathbb{P}(\bm{Z}^\mathcal{T})$ will be better aligned, as shown in Fig.~\ref{fig:insight}(c).



\subsection{Putting Together}
%
The total loss of \modelname~could be obtained by combining the losses of the rating reconstruction module and the embedding alignment module.
%
That is, the loss of \modelname~is given as:
\begin{equation}
\begin{aligned}
L_{\modelname} = L_R + \lambda_L L_{LA} + \lambda_G L_{GA},
\end{aligned}
\end{equation}
where $\lambda_{L}$ and $\lambda_{G}$ are hyper-parameters to balance different type of losses. 
%
In the test phase, one can predict the missing ratings by $\hat{\bm{X}}^\mathcal{S} = D_\mathcal{S}(E_\mathcal{S}(\bm{X}^\mathcal{S}))$ and $\hat{\bm{X}}^\mathcal{T} = D_\mathcal{T}(E_\mathcal{T}(\bm{X}^\mathcal{T}))$ in the source and target domains.
%
% Meanwhile one can predict the missing ratings across domains for cold-start recommendation by $\tilde{\bm{X}}^\mathcal{T} = D_\mathcal{T}(E_\mathcal{S}(\bm{X}^\mathcal{S}))$ or $\tilde{\bm{X}}^\mathcal{S} = D_\mathcal{S}(E_\mathcal{T}(\bm{X}^\mathcal{T}))$.






